Security Assessment and Impact Analysis of Cyberattacks in Integrated T&D Power Systems

In this paper, we examine the impact of cyberattacks in an integrated transmission and distribution (T&D) power grid model with distributed energy resource (DER) integration. We adopt the OCTAVE Allegro methodology to identify critical system assets, enumerate potential threats, analyze, and prioritize risks for threat scenarios. Based on the analysis, attack strategies and exploitation scenarios are identified which could lead to system compromise. Specifically, we investigate the impact of data integrity attacks in inverted-based solar PV controllers, control signal blocking attacks in protective switches and breakers, and coordinated monitoring and switching time-delay attacks.

==> 6-review.tex <==
\newpage \onecolumn 

\fontfamily{bch}\selectfont 

\null\vspace{2cm}
\noindent Dear Associate Editor and Reviewers,\\ 

\noindent We appreciate your constructive  comments on our work and we would like to
thank you for the valuable feedback about our submission to the \textit{2021 IEEE Power \& Energy Society General Meeting}. Please find an updated version of our manuscript that has been revised accordingly.\\

\noindent The main changes to the revised manuscript are as follows: 
\begin{itemize}
\item We have edited the manuscript bibliography and section headings following the PESGM template;

\item We have revised the Conclusions section of the paper to emphasize the main findings of this research work;

\item {We have included clarifications regarding the placement and design characteristics of some vulnerable power system components, to elucidate how they can potentially affect the overall system operation.}\\
\end{itemize}
 
\noindent Our complete and detailed comments on your specific points are following in {\em italics}. We have attempted to address all the issues in this revised manuscript.\\

%\noindent 
%All modifications performed on the manuscript are highlighted in {\color{blue} blue color}.
 
~\newline
Kind regards,
\vspace{10pt}

\noindent Ioannis Zografopoulos, Charalambos Konstantinou, Nektarios Georgios Tsoutsos, Dan Zhu and Robert Broadwater 

\newpage



\begin{center}
\large {\bf Reviewer 1}
\end{center}

\noindent{\bf Q-R1.1: Template Modification: Bibliography should change according to the PESGM template; hyperlinks should be removed; and the subsection headlines should follow the PESGM template.
}

\vspace{5pt}
\noindent{\em {\bf A-R1.1:} We thank the reviewer for the suggestions. 

\vspace{5pt}
We have edited the bibliography to follow the PES notation and have removed any hyperlinks included in the references. We have also revised the manuscript and modified any subsection headlines that were not following the PES template.}

\vspace{20pt}
\noindent{\bf Q-R1.2: The conclusion section should provide the most important finding of the study not only provide a summary of the manuscript.
}

\vspace{5pt}
\noindent{\em {\bf A-R1.2:} We thank the reviewer for the insightful comment. We have edited the conclusion section accordingly to reflect the motivation and the most crucial observation of our analysis. The updated Conclusions section is the following.

\vspace{5pt}

\textit{``In this paper, we demonstrate how simulation-aware risk assessment analyses are critical for identifying vulnerable grid components. The security enhancement of such components could lead to more resilient power systems against cyberattacks. An integrated T\&D system model is used for the attack simulations, and the OCTAVE Allegro methodology is utilized for the risk assessment process.''}}

\vspace{20pt}


\begin{center}
\large {\bf Reviewer 2}
\end{center}

\noindent{\bf Q-R2.1: The thematic is interesting, but the authors lack in showing the originality and innovation of this paper.
}

\vspace{5pt}
\noindent{\em {\bf A-R2.1:} We greatly appreciate the reviewer for the comment about the thematic of the paper. We have carefully revised the paper to demonstrate its originality as well as illustrate the importance of simulation-aided risk assessment of power systems using the OCTAVE Allegro methodology. %Once again, we thank the reviewer for allowing us to improve our work using their useful comments.
}

\vspace{20pt}

\newpage

\begin{center}
\large {\bf Reviewer 3}
\end{center}

\noindent{\bf Q-R3.1: It is interesting to observe that breaker 2 is the most vulnerable device. The location of breaker 1 is similar to breaker 2 from Fig. 3. The distance to a genset are the same observed from Fig. 4. It would be great if there is a further discussion on the result. More details about the case such as the size of the generators at each breaker maybe helpful. In addition, the impact of a cyber attack is measured by the number of violations. It would be good to have a further discussion between the number of violations to more direct impacts such as load losses, device failures or blackouts. }

\vspace{5pt}
\noindent{\em {\bf A-R3.1:} We thank the reviewer for the excellent question and the on-point observations.

\vspace{5pt}

Fig. 3 serves only as a simplified pictorial representation of the integrated T\&D. It does not reflect the actual grid interconnections and any topology assumptions based on Fig. 3 can be inaccurate. For confidentiality and security reasons, the integrated T\&D system model topology cannot be disclosed. Similarly, the nameplate capacities of generators, number of connected residential/commercial loads, microgrid characteristics, power flows, etc. cannot be provided since they would expose the actual power system architecture. Thus, we have sanitized the results of our analysis in order to delineate the useful information, without open sourcing intelligence for the critical infrastructure which, if maliciously exploited, could endanger the power grid.

Furthermore, although Fig. 4 illustrates that breakers 1 and 2 are at similar distances from their gensets, the number of their corresponding violations is significantly larger. This observation dictates that breaker 2 is supporting more loads (out of which some might be critical loads, thus ``non-shedable''). Furthermore, the increased number of violations also factors that in the event of a breaker 2 trip, the loads that do not belong to microgrids (able to operate autonomously and meet the power demand) will have to be supplied from neighbouring resources. Altering power dispatch to accommodate for such unexpected power increase leads to uneconomical grid operation, and thus, more violations. For our case study, the number of violations serves as an ``performance indicator'' of ``penalty metric'', given that specific system information cannot be disclosed, i.e., more violations outline worse grid operation conditions.

The goal of our analysis is to demonstrate that simulation-aided risk assessment can be a useful tool for ISOs and DSOs. It can serve as a framework to discover power system vulnerabilities, design mitigation strategies to counter them, and support redundancy measures to overcome cyberattacks or unexpected failures. Our methodology serves as a proof-of-concept in this direction, and as such the violation terminology can assume different meanings depending on the type of analysis being conducted. For example, violations could mean number of compromised/offline devices, overloaded lines, etc. if we are simulating a DoS attack scenario. On the other hand, it could also mean that the electricity price has surpassed a certain threshold if we are conducting a false-data-injection attack (FDIA) study, where the attacker aims to spoof the locational marginal price (LMP) mechanism leading to financial misconduct or uneconomic grid operation.
}

